MAGIC: Detecting Advanced Persistent Threats via Masked Graph Representation Learning

Advance Persistent Threats (APTs), adopted by most delicate attackers, are becoming increasing common and pose great threat to various enterprises and institutions. Data provenance analysis on provenance graphs has emerged as a common approach in APT detection. However, previous works have exhibited several shortcomings: (1) requiring attack-containing data and a priori knowledge of APTs, (2) failing in extracting the rich contextual information buried within provenance graphs and (3) becoming impracticable due to their prohibitive computation overhead and memory consumption. In this paper, we introduce MAGIC, a novel and flexible self-supervised APT detection approach capable of performing multi-granularity detection under different level of supervision. MAGIC leverages masked graph representation learning to model benign system entities and behaviors, performing efficient deep feature extraction and structure abstraction on provenance graphs. By ferreting out anomalous system behaviors via outlier detection methods, MAGIC is able to perform both system entity level and batched log level APT detection. MAGIC is specially designed to handle concept drift with a model adaption mechanism and successfully applies to universal conditions and detection scenarios. We evaluate MAGIC on three widely-used datasets, including both real-world and simulated attacks. Evaluation results indicate that MAGIC achieves promising detection results in all scenarios and shows enormous advantage over state-of-the-art APT detection approaches in performance overhead.

==> examples/figures.tex <==
%-------------------------------------------------------------------------------
\section{Floating Figures and Lists}
\label{sec:figs}
%-------------------------------------------------------------------------------


%---------------------------
\begin{figure}
\begin{center}
\begin{tikzpicture}
  \draw[thin,gray!40] (-2,-2) grid (2,2);
  \draw[<->] (-2,0)--(2,0) node[right]{$x$};
  \draw[<->] (0,-2)--(0,2) node[above]{$y$};
  \draw[line width=2pt,blue,-stealth](0,0)--(1,1)
        node[anchor=south west]{$\boldsymbol{u}$};
  \draw[line width=2pt,red,-stealth](0,0)--(-1,-1)
        node[anchor=north east]{$\boldsymbol{-u}$};
\end{tikzpicture}
\end{center}
\caption{\label{fig:vectors} Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. }
\end{figure}
%% %---------------------------


Here's a typical reference to a floating figure:
Figure~\ref{fig:vectors}. Floats should usually be placed where latex
wants then. Figure\ref{fig:vectors} is centered, and has a caption
that instructs you to make sure that the size of the text within the
figures that you use is as big as (or bigger than) the size of the
text in the caption of the figures. Please do. Really.

In our case, we've explicitly drawn the figure inlined in latex, to
allow this tex file to cleanly compile. But usually, your figures will
reside in some file.pdf, and you'd include them in your document
with, say, \textbackslash{}includegraphics.

Lists are sometimes quite handy. If you want to itemize things, feel
free:

\begin{description}
  
\item[fread] a function that reads from a \texttt{stream} into the
  array \texttt{ptr} at most \texttt{nobj} objects of size
  \texttt{size}, returning returns the number of objects read.

\item[Fred] a person's name, e.g., there once was a dude named Fred
  who separated usenix.sty from this file to allow for easy
  inclusion.
\end{description}

\noindent
The noindent at the start of this paragraph in its tex version makes
it clear that it's a continuation of the preceding paragraph, as
opposed to a new paragraph in its own right.

\subsection{LaTeX-ing Your TeX File}
%-----------------------------------

People often use \texttt{pdflatex} these days for creating pdf-s from
tex files via the shell. And \texttt{bibtex}, of course. Works for us.


==> letter_figure_table/fig_ablation_0_revised.tex <==
\begin{figure}[t]
    \centering
    \subfigure[FR, on Wget dataset]{\includegraphics[width=0.495\hsize]{tex_figure/imgs_revised/ablation_fr.pdf}\label{fig_ablation_fr_letter}}
    \subfigure[SR, on Wget dataset]{\includegraphics[width=0.495\hsize]{tex_figure/imgs_revised/ablation_sr.pdf}\label{fig_ablation_sr_letter}}
    \caption{Effect of different reconstruction components on \system{}'s performance and efficiency.}
    \label{fig_ablation_revised_letter}
\end{figure}

==> letter_figure_table/fig_ablation_revised.tex <==
\begin{figure*}[t]
    \centering
    \setcounter{subfigure}{0}
    \subfigure[\textbf{\emph{d}}, on Wget dataset]{\includegraphics[width=0.330\hsize]{tex_figure/imgs_revised/ablation_d.pdf}\label{fig_d_revised_letter}}
    \subfigure[\textbf{\emph{l}}, on Wget dataset]{\includegraphics[width=0.330\hsize]{tex_figure/imgs_revised/ablation_l.pdf}\label{fig_l_revised_letter}}
    \subfigure[\textbf{\emph{r}}, on Wget dataset]{\includegraphics[width=0.330\hsize]{tex_figure/imgs_revised/ablation_r.pdf}\label{fig_r_revised_letter}}
    \caption{Effect of different hyper-parameters on \system{}'s performance and efficiency.}
    \label{fig_hyperparameter_letter}
\end{figure*}

==> letter_figure_table/fig_case_revised.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{tex_figure/imgs_revised/motivation2.pdf}
    \caption{Another provenance graph of our motivating example (i.e. Pine Backdoor). Red nodes represent ground-truth malicious entities and black nodes are benign ones. Numbers assigned to nodes are their corresponding anomaly scores, assessed by \system{}'s detection module.}
    \label{fig_case_revised_letter}
\end{figure}

==> letter_figure_table/fig_gc_revised.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.495\textwidth]{tex_figure/imgs_revised/gc.pdf}
    \caption{Example of \system{}'s graph construction steps.}
    \label{fig_gc_revised_letter}
  \end{figure}

==> letter_figure_table/fig_motivation_revised.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.495\textwidth]{tex_figure/imgs_revised/motivation1.pdf}
    \caption{The provenance graph of a real-world APT attack, exploiting the Pine Backdoor vulnerability. All attack-irrelevant entities and interactions have been removed from the provenance graph.}
    \label{fig_motivation_revised_letter}
  \end{figure}

==> letter_figure_table/fig_overview_revised.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\hsize]{tex_figure/imgs_revised/model.pdf}
    \caption{Overview of \system{}'s detection pipeline.}
    \label{fig_overview_revised_letter}
  \end{figure*}

==> letter_figure_table/fig_score.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{tex_figure/imgs_revised/score.pdf}
    \caption{Distribution of anomaly scores of both benign and malicious entities, tested on all datasets.}
    \label{fig_score_revised_letter}
\end{figure}

==> letter_figure_table/tab_adversarial.tex <==
\begin{table}[t]
\centering
\small
\setlength{\belowcaptionskip}{0.2cm}
\caption{Impact of different adversarial attack strategies on \system{}'s detection effectiveness.}
\label{tab_adversarial_letter}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Attack Type & None & MFE & MSE & MCE & BFP \\
\hline

AUC & 0.9999 & 0.9999 & 0.9999 & 0.9994 & 0.9942\\
\hline
\end{tabular}
\end{table}

==> letter_figure_table/tab_compare_result_revised.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Comparison between \system{} and state-of-the-art APT detection methods on different datasets. Within column \emph{supervision}, B indicates benign data, A refers to attack data and SA for streaming attack data.}
\label{tab_compare_result_revised_letter}

\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}

\hline
Dataset & Approach & Train Ratio & Supervision & Precision &  F1-Score & Recall & FPR\\
\hline\hline

\multirow{5}{*}{StreamSpot} & StreamSpot & 80\% & B & 73\% & 81\% & 91\% & 6.6\%\\

 & Unicorn (baseline) & 75\% & B & 95\% & 96\% & 93\% & 1.6\%\\

 & Prov-Gem & 80\% & B,A & 100\% & 97\% & 94\% & \textbf{0\%}\\

 & ThreaTrace & 75\% & B & 98\% & 99\% & 99\% & 0.4\%\\

 & \textbf{\system{} (Ours)} & 80\% & B & 99\% & \textbf{99\%} & \textbf{100\%} & 0.6\%\\
\hline\hline

\multirow{4}{*}{\makecell[c]{Unicorn\\Wget}} & Unicorn (baseline) & 80\% & B & 86\% & 90\% & 95\% & 15.5\%\\

 & Prov-Gem & 80\% & B,A & 100\% & 89\% & 80\% & \textbf{0\%}\\

 & ThreaTrace & 80\% & B & 93\% & 95\% & \textbf{98\%} & 7.4\%\\

 & \textbf{\system{} (Ours)} & 80\% & B & 98\% & \textbf{97\%} & 96\% & 2.0\%\\
\hline\hline

\multirow{5}{*}{\makecell[c]{DARPA\\E3 Trace}} & DeepLog & N/A & B,A & 41\% & 51\% & 68\% & 2.7\%\\

& Log2vec (baseline) & N/A & B,A & 54\% & 64\% & 78\% & 1.8\%\\

& ThreaTrace & N/A & B & 72\% & 83\% & 99\% & 1.1\%\\

& ShadeWatcher & 80\% & B,SA & 97\% & 99\% & \textbf{99\%} & 0.3\%\\

 & \textbf{\system{} (Ours)} & 80\% & B & \textbf{99\%} & \textbf{99\%} & 99\% &\textbf{0.1\%}\\
\hline\hline

\multirow{4}{*}{\makecell[c]{DARPA\\E3 THEIA}} & DeepLog & N/A & B,A & 16\% & 15\% & 14\% & 0.5\%\\

& Log2vec (baseline) & N/A & B,A & 62\% & 64\% & 66\% & 0.3\%\\

& ThreaTrace & N/A & B & 87\% & 93\% & 99\% & \textbf{0.1\%}\\

 & \textbf{\system{} (Ours)} & 80\% & B & \textbf{98\%} & \textbf{99\%} & \textbf{99\%} & 0.1\%\\
\hline\hline

\multirow{4}{*}{\makecell[c]{DARPA\\E3 CADETS}} & DeepLog & N/A & B,A & 23\% & 35\% & 74\% & 4.4\%\\

& Log2vec (baseline) & N/A & B,A & 49\% & 62\% & 85\% & 1.6\%\\

& ThreaTrace & N/A & B & 90\% & 95\% & \textbf{99\%} & 0.2\%\\

 & \textbf{\system{} (Ours)} & 80\% & B & \textbf{94\%} & \textbf{97\%} & 99\% & \textbf{0.2\%}\\
\hline
\end{tabular}
}
\end{table}


==> letter_figure_table/tab_entity_dataset_revised.tex <==
\begin{table}[t]
\caption{Datasets for System Entity Level Detection.}
\label{tab_entity_dataset_revised_letter}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Dataset & Scenario & Malicious &\#Node &\#Edge & Size (GB)\\
\hline\hline
 \multirow{4}{*}{DARPA E3 Trace} & Benign & & 3,220,594 & \multirow{4}{*}{4,080,457} & \multirow{4}{*}{15.40}\\

 & Extension Backdoor & \checkmark & 732 & & \\

 & Pine Backdoor & \checkmark & 67,345 & & \\

 & Phishing Executable & \checkmark & 5 & & \\
 \hline\hline
 \multirow{2}{*}{DARPA E3 THEIA} & Benign & & 1,598,647 & \multirow{2}{*}{2,874,821} & \multirow{2}{*}{17.91}\\

 & Attack & \checkmark & 25,319 & & \\
\hline\hline
\multirow{2}{*}{DARPA E3 CADETS} & Benign & & 1,614,189 & \multirow{2}{*}{3,303,264} & \multirow{2}{*}{18.38}\\

 & Attack & \checkmark & 12,846 & & \\
\hline
\end{tabular}
}
\end{table}


==> letter_figure_table/tab_general_result_revised.tex <==
\begin{table*}[t]
\caption{\system{}'s detection results on different datasets. For batched log level detection, the detection targets are log pieces. And for system entity level detection, system entities are the targets.}
\label{tab_general_result_revised_letter}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Granularity} & \multicolumn{2}{c|}{\multirow{2}{*}{Dataset}} & \multirow{2}{*}{Train Ratio} & \multicolumn{2}{c|}{Ground Truth} &\multirow{2}{*}{\#TP} &\multirow{2}{*}{\#FP} & \multirow{2}{*}{\#TN} & \multirow{2}{*}{\#FN} & \multirow{2}{*}{Precision} & \multirow{2}{*}{Recall} & \multirow{2}{*}{FPR} & \multirow{2}{*}{F1-Score} & \multirow{2}{*}{AUC}\\
\cline{5-6}

 & \multicolumn{2}{c|}{} & & \#Benign & \#Malicious & & & & & & & & &\\
\hline\hline
 
 \multirow{2}{*}{Batched log level} & \multicolumn{2}{c|}{StreamSpot} & 80\% & 100 & 100 & 100.0 & 0.59 & 99.41 & 0.0 & 99.41\% & 100.00\% & 0.59\% & 99.71\% & 99.95\%\\
 \cline{2-15}

 & \multicolumn{2}{c|}{Unicorn Wget} & 80\% & 25 & 25 & 24.0 & 0.5 & 24.5 & 1.0 & 98.02\% & 96.00\% & 2.00\% & 96.98\% & 96.32\%\\
 \hline\hline

 \multirow{6}{*}{System entity level} & \multirow{4}{*}{DARPA E3 Trace} & All & \multirow{4}{*}{80\%} & \multirow{4}{*}{616,025} & 68,082 & 68,072 & \multirow{4}{*}{569} & \multirow{4}{*}{615,456} & 10 & \multirow{4}{*}{99.17\%} & \multirow{4}{*}{99.98\%} & \multirow{4}{*}{0.09\%} & \multirow{4}{*}{99.57\%} & \multirow{4}{*}{99.99\%}\\
 \cline{3-3}\cline{6-7}\cline{10-10}

 & & Extension Backdoor & & & 732 & 727 & & & 5 & & & & &\\
 \cline{3-3}\cline{6-7}\cline{10-10}

 & & Pine Backdoor & & & 67,345 & 67,342 & & & 3 & & & & &\\
 \cline{3-3}\cline{6-7}\cline{10-10} 

 & & Phishing Executable & & & 5 & 3 & & & 2 & & & & &\\
 \cline{2-15}

 & DARPA E3 THEIA & All & 80\% & 319,448 & 25,319 & 25,318 & 456 & 318,992 & 1 & 98.23\% & 99.99\% & 0.14\% & 99.11\% & 99.87\%\\
 \cline{2-15}

 & DARPA E3 CADETS & All & 80\% & 344,327 & 12,846 & 12,816 & 759 & 343,568 & 30 & 94.40\% & 99.77\% & 0.22\% & 97.01\% & 99.77\%\\
 \hline

\end{tabular}}
\end{table*}


==> tex_figure/fig_ablation.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[\textbf{\emph{d}}, on Wget dataset]{\includegraphics[width=0.245\hsize]{tex_figure/imgs/d.pdf}\label{fig_d}\label{fig_ablation_1}}
    \subfigure[\textbf{\emph{l}}, on Wget dataset]{\includegraphics[width=0.245\hsize]{tex_figure/imgs/l.pdf}\label{fig_l}\label{fig_ablation_2}}
    \subfigure[\textbf{\emph{r}}, on Wget dataset]{\includegraphics[width=0.245\hsize]{tex_figure/imgs/r.pdf}\label{fig_r}\label{fig_ablation_3}}
    \subfigure[\textbf{\emph{$\theta$}}, on all datasets]{\includegraphics[width=0.245\hsize]{tex_figure/imgs/theta.pdf}\label{fig_ts}\label{fig_ablation_4}}
    \label{fig_ablation}
    \caption{Example of \system{}'s graph construction steps.}
\end{figure*}

==> tex_figure/fig_case.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{tex_figure/imgs/motivation2.pdf}
    \caption{Another provenance graph of our motivating example(i.e. Pine Backdoor). Red nodes represent ground-truth malicious entities and black nodes are benign ones. Numbers assigned to nodes are their corresponding anomaly scores, assessed by \system{}'s detection module.}
    \label{fig_case}
\end{figure}

==> tex_figure/fig_gmae.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{tex_figure/imgs/gmae.pdf}
    %\caption{Architecture of \system{}'s graph representation \system{}.}
    \caption{Graph representation module of \system{}.}
    \label{fig_gmae}
  \end{figure}

==> tex_figure/fig_motivation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{tex_figure/imgs/motivation1.pdf}
    \caption{The provenance graph of a real-world APT attack, exploiting the Pine Backdoor vulnerability. All attack-irrelevant entities and interactions have been removed from the provenance graph.}
    \label{fig_motivation}
  \end{figure}

==> tex_figure/fig_overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics{tex_figure/imgs/model.pdf}
    \caption{Overview of \system{}'s detection pipeline.}
    \label{fig_overview}
  \end{figure*}

==> tex_figure/fig_roc.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{tex_figure/imgs/roc.pdf}
    \caption{ROC curves on all datasets.}
    \label{fig_roc}
  \end{figure}

==> tex_figure/fig_scatter.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.50\textwidth]{tex_figure/imgs/scatter.pdf}
    \caption{Latent space of system state embeddings in the StreamSpot dataset. Each point represents a log piece in the dataset, which belongs to one of six scenarios: watching YouTube, checking G-mail, playing vgame, undergoing a driven-by-download attack, downloading ordinary files and watching CNN.}
    \label{fig_scatter}
  \end{figure}

==> tex_section/discussion.tex <==
\section{Discussion and Limitations}\label{sec_discussion}

\noindent\textbf{Quality of training data.} \system{} models benign system behaviors and detect APTs with outlier detection. Similar to other anomaly-based APT detection approaches\cite{aptlearnbased-10,aptstatbasednodoze-7, aptstatbased-8}, we assume that all up-to-date benign system behaviors are observed during training log collection. However, if \system{} is trained with low quality data that insufficiently covers system behaviors, many false positives can be generated. 

Another problem regarding the training data is that we assume APT attacks do not penetrate the logging system, which is not true in real-world settings. However, recent works show that the reliability of system audit logs can be ensured in various ways, e.g. secure logging systems\cite{securelog1-45,securelog2-46} and system hardening. With these techniques involved, \system{} is able to perform APT detection on tamper-free audit logs.

\noindent\textbf{Outlier Detection.} \system{} implemented a KNN-based outlier detection module for APT detection. While our detection module completes training and inference in logarithmic time, its efficiency on large datasets is still unsatisfactory. To illustrate, our detection module takes 10.5 minutes to check 1,200,000 targets, making up 98\% of total inference time. Other outlier detection methods, such as One-class SVM\cite{ocsvm-47} and Isolation Forest\cite{if-48}, do not fit in our detection setting and cannot adapt to concept drift. It is possible that cluster-based detection methods are more suitable to huge datasets and our KNN-based method can be extended to GPU usage with python library CUML and FAISS. We leave such improvements on our detection module to future research.

\noindent\textbf{Targeted Attacks.} In Sec. \ref{sec_evaluation_2}, we show that \system{} handles stealth attacks well, which avoid detection by behaving similar to the benign system. However, if attackers get to know how \system{} work in details, they might conduct elaborately designed attacks to infiltrate our detector. We provide a detailed example of such targeted attack and our corresponding countermeasure in Appendix \ref{appe_c}. As GNN-based methods become increasingly popular and powerful in APT detection, designing and avoiding those targeted attacks on the GNNs stands for an interesting research topic.



==> tex_section/evaluation.tex <==
\section{Evaluation}\label{sec_evaluation}

We use 93GB of audit logs derived from various system auditing softwares to evaluate the effectiveness and efficiency of \system{}. We first describe our experimental settings(Sec. \ref{sec_evaluation_1}), then elaborate the effectiveness of \system{} in different scenarios(Sec. \ref{sec_evaluation_2}), conduct a false positive analysis and assess the usefulness of the model adaption mechanism(Sec. \ref{sec_evaluation_3}) and an ablation study on the components of \system{}(Sec. \ref{sec_evaluation_4}). The run-time performance overhead of \system{} is analyzed in Sec. \ref{sec_evaluation_5}. In addition, a detailed case study on our motivation example is conducted in Sec. \ref{sec_evaluation_6} to illustrate how \system{}'s pipeline work for APT detection. These experiments are performed on a linux desktop computer with an Intel Core i7-12700K CPU, 32GB physical memory and a NVIDIA RTX 3090 GPU.

\subsection{Experimental Settings}\label{sec_evaluation_1}
We evaluate the effectiveness of \system{} on three public datasets: the StreamSpot dataset\cite{streamspotdataset-21} the Unicorn Wget dataset\cite{unicorndataset-22} and the DARPA TRACE dataset\cite{darpadataset-20}. These datasets vary in volume, origin and granularity. We believe by testing \system{}'s performance on these datasets, we are able to compare \system{} with as many \emph{state-of-the-art} APT detection approaches as possible and explore the universality and applicability of \system{}. we provide detailed descriptions of the three datasets as follows.

\noindent\textbf{StreamSpot Dataset.} The StreamSpot dataset(See Table \ref{tab_batched_dataset}) is a simulated dataset collected and made public by StreamSpot\cite{streamspot-35} using auditing system SystemTap\cite{systemtap-41}. The StreamSpot dataset contains 600 pieces of audit logs monitoring system calls under 6 unique scenarios. Five of those scenarios are simulated benign user behaviors, including watching videos online, downloading from websites and checking e-mails while the attack scenario simulates a driven-by-download attack. The dataset contains an average 149,618 log entries per piece and is considered a relatively small dataset. Since no labels of log entries and system entities are provides, we perform \emph{batched log level detection} on the StreamSpot dataset similar to previous works\cite{aptlearnbased-10,aptlearnbasedprovgem-15,aptlearnbasedthreatrace-17}.

\input{tex_table/tab_batched_dataset.tex}
\noindent\textbf{Unicorn Wget Dataset.} The Unicorn Wget dataset(See Table \ref{tab_batched_dataset}) contains simulated attacks designed by Unicorn\cite{aptlearnbased-10}. Specifically, it contains 150 pieces of logs collected with Camflow\cite{camflow-34}, where 125 of them are collected from benign scenarios and 25 of them contains a \emph{supply-chain attack}. Those attacks, known as stealth attacks, are elaborately designed by the Unicorn team to behave similar to benign system workflows. Also, attackers in these scenarios skip the \emph{reconnaissance} phase of typical APT attacks\cite{killchain-42}, making them even more difficult to identify. The Unicorn Wget dataset is considered the hardest among our experimental dataset for its huge volume, complicated log format and the similarity between benign and malicious system behaviors. The same as state-of-the-art approaches, we perform \emph{batched log level detection} on this dataset.

\noindent\textbf{DARPA TRACE Dataset.} The DARPA TRACE dataset(See Table \ref{tab_entity_dataset}), as a part of the DARPA Transparent Computing dataset, is collected among an enterprise network during an adversarial engagement. APT attacks exploiting different vulnerabilities\cite{darpadataset-20} are conducted by the red team during the engagements, aiming to exfiltrate sensitive information. Blue teams, including the TRACE team, try to identify those APT attacks by collecting audit logs from network hosts and performing causality analysis on them. The DARPA TRACE dataset consists of 15.0GB of well-labeled records, containing as many as 6,113,983 system entities and 22,161,538 interactions. Thus, we evaluate \system{}'s effectiveness of \emph{system entity level detection} and address the overhead issue on DARPA TRACE dataset.

\input{tex_table/tab_entity_dataset.tex}
For different dataset,we employed different dataset splits to evaluate the model and we use only benign samples for training. For the StreamSpot dataset, we randomly choose 400 pieces of benign logs for training and the rest 200 pieces for testing, resulting in an balanced test set. For the Unicorn Wget dataset, 100 pieces of benign logs are selected for training while the rest are for testing, the same as conducted in Unicorn. For the DARPA TRACE dataset, we split log entries according to their order of occurrence. The earliest 20\% of the log entries are selected as the training set while the rest 80\% are preserved for testing. During evaluation, the average performance of \system{} under 100 global random seeds is reported as the final result.

\subsection{Effectiveness}\label{sec_evaluation_2}
\system{}'s effectiveness in multi-granularity APT detection is evaluated on three datasets. Here we present the detection results of \system{} on each dataset, then compare it with state-of-the-art APT detection approaches on those datasets.

\noindent\textbf{Detection Result.} Results show that \system{} successfully detect APTs with high accuracy in different scenarios. We present the detection results of \system{} on each dataset in Table \ref{tab_general_result} and their corresponding ROC curves in Figure \ref{fig_roc}.

\input{tex_table/tab_general_result.tex}
\input{tex_figure/fig_roc.tex}
On easy datasets such as the StreamSpot dataset, \system{} achieves almost perfect detection results. This is because the StreamSpot dataset collects only single user activity per log piece, resulting in system behaviors that can be easily separated from each other. We further present this effect by visualizing the distribution of system state embeddings abstracted from those log pieces in Figure \ref{fig_scatter}. The system state embeddings are clearly separated into 6 categories, perfectly matching the 6 scenarios involved in the dataset. Also, this indicates that \system{}'s graph representation module excels at abstracting system behaviors into such embeddings.

\input{tex_figure/fig_scatter.tex}
When dealing with the Unicorn Wget dataset, \system{} yields an average 98.01\% precision and 96.00\% recall, significantly lower compared to that of the StreamSpot dataset. \system{}'s self-supervised style makes it difficult to distinguish between stealth attacks and benign system behaviors. However, \system{} still successfully recovers an average 24 out of 25 log pieces with only 0.5 false positives generated, better than any of the state-of-the-art detectors.

On the DARPA TRACE dataset, \system{} achieves an average 99.94\% recall and 0.509\% false positive rate with only 20\% log entries for training. This indicates \system{} quickly learns to model system behaviors with a small proportion of benign logs. The test set in this scenario is unbalanced, which means the total number of ground-truth benign entities far exceeds that of malicious entities. Specifically, only 68,265 of 4,842,212 test entities are labeled malicious. However, few false positives are generated, as \system{} identifies malicious entities with outlier detection methods and anomalous entities are naturally detected as abnormalities.

\noindent\textbf{\system{} vs. \emph{State-of-the-art}.} 
The three datasets used to evaluate \system{} are also used by several state-of-the-art learning-based APT detection approaches. For instance, Unicorn\cite{aptlearnbased-10}, Prov-Gem\cite{aptlearnbasedprovgem-15} and ThreaTrace\cite{aptlearnbasedthreatrace-17} for Unicorn Wget and StreamSpot dataset, ThreaTrace and ShadeWatcher\cite{aptlearnbasedshadewatcher-18} for DARPA TRACE dataset. Methods that require \emph{a priori} information about APTs, such as Holmes\cite{aptrulebasedholmes-3}, Poirot\cite{aptrulebased-5} and Morse\cite{aptrulebased-6}, are not taken into consideration as \system{} cannot be compared to them in the same detection scenario.

Comparison results between \system{} and other state-of-the-art approaches on each dataset is presented in Table \ref{tab_compare_result}. Comparison between \system{} and other unsupervised approaches(i.e. Unicorn and ThreaTrace) yields a total victory of our approach, revealing \system{}'s effectiveness in modeling and detecting outliers of benign system behaviors with no supervision from attack-containing logs. 

\input{tex_table/tab_compare_result.tex}
Beyond unsupervised methods, Prov-Gem is a supervised APT detector based on GATs. However, it failed to achieve a better detection result on even the easiest StreamSpot dataset. This is mainly because simple GAT layers supervised on classification tasks are not as expressive as graph masked auto-encoders in producing high-quality graph embeddings. Another APT detector mentioned, ShadeWatcher, adopts a semi-supervised detection approach. ShadeWatcher leverages TransR\cite{transr-43} and graph neural networks(GNNs) to detect APTs based on recommendation and is able to achieve the best detection result on DARPA TRACE dataset. TransR, a self-supervised graph representation method on Knowledge Graphs, contributes most to the extraordinary performance of ShadeWatcher. Unfortunately, TransR is extremely expensive in computation overhead. For example, ShadeWatcher spends as much as 12 hours training the TransR module on DARPA TRACE dataset. On the contrary, evaluation on the computation overhead of \system{}(Sec.\ref{sec_evaluation_5}) shows that \system{} is able to complete training on same amount of training data 90 times faster than ShadeWatcher.


\subsection{False Positive Analysis}\label{sec_evaluation_3}

For real-time applications, APT detectors must prevent false alarms at best effort, as those false alarms often tire and confuse security analysts. We evaluate \system{}'s false positive rate on benign audit logs and investigate how our model adaption mechanism reduces those false alarms. Table \ref{tab_fp_result} shows \system{}'s false positive rate on each dataset. Within each dataset, only benign logs are used for training and testing. \system{} yields low false positive rates(around 0.5\%) with large training data. This is because \system{} models benign system behaviors with self-supervised graph embeddings, allowing it to effectively handle unseen system entities and measure the similarity between them and benign behaviors. 

Our model adaption mechanism is designed to help \system{} learn from newly-observed unseen behaviors. We evaluate how such mechanism reduces false positives on benign audit logs in Table \ref{tab_fp_result}. Specifically, we tested the performance of \system{} on DARPA TRACE dataset under five different settings:

\vspace{3pt}\noindent$\bullet$~Training on the first 20\% log entries and testing on the rest 80\% with no adaption, identical to our original setting.

\vspace{3pt}\noindent$\bullet$~Training on the first 20\% and testing on the last 60\% with no adaption, for comparison purpose.

\vspace{3pt}\noindent$\bullet$~Training on the first 20\%, adapting on false positives generated from the following 10\%, and testing on the last 60\%.

\vspace{3pt}\noindent$\bullet$~Training on the first 20\%, adapting on false positives generated from the following 20\%, and testing on the last 60\%.

\vspace{3pt}\noindent$\bullet$~Training on the first 20\%, adapting on both false positives and true negatives generated from the following 20\% log entries, and testing on the last 60\%.

\input{tex_table/tab_fpr.tex}
Experimental results indicates that adapting the model to reported false positives consistently reduce the number of false positives by 11.0\%. A further 1\% reduction is achieved by feeding both false positives and true negatives to the model. This is because the graph representation module can be retrained with any data to enhance its representation ability, as described in Sec \ref{sec_model_4}. 

\subsection{Ablation Studies}\label{sec_evaluation_4}
\system{} is a three-step APT detection approach that consists of a graph representation module and a detection module, where the graph representation module is trained upon masked feature reconstruction and sample-based structure reconstruction. In this section, we first address the effectiveness of important individual components and reconstruction techniques, then carry out a hyper-parameter analysis to evaluate the sensitivity of \system{}. The individual component analysis is conducted on the most difficult Wget dataset and the hyper-parameter analysis is conducted on all datasets.

\noindent\textbf{Effect of Masked Feature Reconstruction.} We study how masked feature reconstruction impact \system{} and Table \ref{tab_ablation} presents the overall performance of \system{} with different feature reconstruction criteria. Results indicates masked feature reconstruction is advantageous than ordinary feature reconstruction by boosting model performance by 1.5\% and reducing training time by 46\% on average. Furthermore, performance comparison between with and without feature reconstruction shows that feature reconstruction acts as the major supervision for our graph representation module.

\noindent\textbf{Effect of Sample-based structure reconstruction.} As described in previous sections, the sample-based structure reconstruction provides a supervision for the graph representation module, enriching the graph embeddings. Effect of such reconstruction is evaluated in Table \ref{tab_ablation}. The sample-based structure reconstruction provides a 7.4\% bonus on model performance. And compared to ordinary structure reconstruction that attempts to reconstruction the whole adjacency matrix, sample-based structure reconstruction speeds up model training by an average 1010\%, preventing Out-of-memory(OOM) problems on huge datasets at the cost of 0.1\% performance.

\input{tex_table/tab_ablation.tex}
\noindent\textbf{Effect of the Graph Representation Module.} The graph representation module extract high-quality graph embeddings from raw provenance graphs ready for subsequent APT detection. We have already assessed the quality of such embeddings in Sec. \ref{sec_evaluation_2}. Here we conduct alternative experiments on those embeddings to reveal the effect of the graph representation module. In the first experiment, we measure the average distance between embeddings of test system entities with learned benign ones. As shown in Table \ref{tab_avg_distance}, malicious system entities are far away from benign embeddings, making them easy to identify. Another experiment replaces the detection module with a supervised linear classifier(e.g. LDA\cite{lda-44}) to illustrate the usefulness of graph embeddings. Results show a 99.16\% precision and a 94.79\% recall, higher than \system{} under unsupervised conditions. This also reveals the possibility to apply \system{} to supervised detection scenarios.

\input{tex_table/tab_avg_distance.tex}
 \noindent\textbf{Hyper-parameter sensitivity.} The function of \system{} is controlled by several hyper-parameters, including an embedding dimension \emph{d}, number of GAT layers \emph{l}, node mask rate \emph{r} and the outlier detection threshold $\theta$. Figure \ref{fig_ablation} illustrates how these hyper-parameters affect model performance.

 \input{tex_figure/fig_ablation.tex}
 Higher model performance is achieved with a larger embedding dimension and more GAT layers by extracting and aggregating more information from more distant neighborhoods, as shown in Subfigure \ref{fig_ablation_1} and \ref{fig_ablation_2}. However, this introduces heavier computation and memory consumption. 
 
 On the other hand, a mask rate of $0.5$ yields best results. This is because \system{} is unable to get sufficient training under a lower mask rate. And under a higher mask rate, node features are severely damaged which prevents \system{} to learn node embeddings via feature reconstruction.

 As presented in \ref{fig_ablation_4}, the detection threshold $\theta$ has little impact on model performance on system entity level detection tasks. A lower $\theta$ naturally generates more false positives, as some unfamiliar system behaviors are detected as outliers. On batched log level detection tasks(e.g. the Unicorn Wget dataset), a threshold between 1.5 and 2 yields best results. Such sensitivity is mainly due to 2 reasons: (1) lack of benign data and (2) closeness between benign and malicious entities involved in a stealth attack.

\subsection{Performance Overhead}\label{sec_evaluation_5}

\system{} is designed to perform APT detection with minimum overhead, granting it applicability under various conditions. \system{} completes its training and inference in logarithmic time and takes up linear space. We provide a detailed analysis of its time and space complexity in Appendix \ref{appe_b}. We further test \system{}'s runtime performance on the largest DARPA TRACE dataset and present its processing time and memory consumption in Table \ref{tab_overhead}.

\input{tex_table/tab_overhead.tex}
\system{} takes on average 2.7 minutes to construct provenance graphs from 15GB of audit logs. \system{}'s training process takes only 12.1 minutes to complete and \system{} takes 8.7 minutes to identify malicious system entities among 1,000,000 targets. In real-world settings, GPUs may not be available at all. We also tested performance of \system{} without the GPU. With only CPUs available, the training phase becomes apparently slower, taking as much as 15.3 minutes to complete. The efficiency of graph construction and outlier detection phase is not affected as they are implemented to perform on CPUs. We also measure the max memory consumption during training and inference. An acceptable 1,202MB of physical memory is occupied during training and 453MB during inference. Such low memory consumption not only prevents OOM problems on huge datasets, but also makes \system{} approachable under tight conditions.

Evaluation results on performance overhead manifest the claim that \system{} is advantageous over other state-of-the-art APT detectors in performance overhead. For instance, ATLAS\cite{aptlearnbasedatlas-11} takes about an hour to train its model on 676MB of audit logs and ShadeWatcher\cite{aptlearnbasedshadewatcher-18} takes 1 day to train on the DARPA TRACE dataset. Compared with ShadeWatcher, \system{} is 22 times faster in training under similar setting(i.e. 80\% log entries for training on DARPA TRACE dataset). 

These evaluation results also illustrate that \system{} is fully practicable in different conditions. Considering the fact that the DARPA TRACE dataset is collected in 2 weeks, 1.37GB of audit logs is produced per day. This means under CPU-only conditions, \system{} takes only 5 minutes to detect APTs from those logs and complete model adaption every day. Such promising efficiency makes \system{} an available choice for individuals and small-size enterprises. For larger enterprises and institutions, they produces audit logs in hundreds of GBs every day\cite{datascale-23}. In this case, efficiency of \system{} can be ensured by training and adapting itself with GPUs and parallelizing the detection module with distributed CPU cores.

\subsection{Case Study}\label{sec_evaluation_6}

\input{tex_figure/fig_case.tex}
We use our motivating example described in Sec. \ref{sec_motivation_1} again to illustrate how \system{} detect APTs from audit logs. 
Our motivating example involves an APT attack: Pine Backdoor, which implants an malicious executable to a host via phishing e-mail, aiming to perform internal reconnaissance and build a silent connection between the host and the attacker. We perform \emph{system entity level detection} on it and obtain real detection results from \system{}. First, \system{} constructs a provenance graph from raw audit logs. We present another example provenance graph in Figure \ref{fig_case} to illustrate, with some benign entities and interactions remain uncut this time. Among them, \emph{tcexec} and \emph{162.66.239.75} are malicious entities while the others are benign ones. The graph representation module then obtains their embeddings via the graphs masked auto-encoder. The embedding of \emph{162.66.239.75} is calculated by propagating and aggregating information from its multi-hop neighborhood to model its interaction behavior with other system entities. For instance, its 2-hop neighborhood is namely \emph{tcexec}, \emph{uname} and other benign IP addresses. The detection module subsequently calculate distances between those embeddings and their k-nearest benign neighbors in the latent space and assigns anomaly scores to them. The two malicious entities are given very high anomaly scores(106.29 and 18.3) that far exceed our detection threshold(10) while others present low abnormality(0.1\textasciitilde1.7). Thus, \system{} successfully detect malicious system entities with no false alarm generated.





==> tex_section/implementation.tex <==
\section{Implementation}

We implement \system{} with about 3,500 lines of code in Python 3.8. We developed several log parsers to cope with different format of audit logs, including a simple StreamSpot format\cite{streamspot-35} and more complex ones such as Camflow\cite{camflow-34}and CDM\cite{cdm-36}. Provenance graphs are constructed using the graph processing library Networkx\cite{networkx-37}. Those provenance graphs are generated and stored into an universal JSON format for the sake of compatibility. The graph representation module is implemented via PyTorch\cite{pytorch-38} and the DGL library\cite{dgl-40} and the detection module is developed with Scikit-learn\cite{sklearn-39}. An Adam optimizer with a weight decay factor of $5\times10^{-4}$ is used to optimize the graph representation module.

For hyper-parameters of \system{}, the scaling factor $\gamma$ in the feature reconstruction loss is set to $3$. Other hyper-parameters are tuned with a simple grid search approach, where the dimension $d$ of graph embeddings are searched in \{16, 32, 64, 128, 256\}, the number of GAT layers $l$ in the graph encoder is chosen in \{1, 2, 3, 4\}, the mask rate of nodes is tuned in \{0.3, 0.5, 0.7\}, the outlier detection threshold $\theta$ between 1 and 10 and the learning rate in \{0.005, 0.001, 0.0005\}. The best detection outcome is achieved with an embedding dimension 256, a four layer graph encoder and a mask rate of 0.5 under a learning rate of 0.005. 

To reduce memory consumption of \system{} on very large datasets(e.g. the DARPA TRACE dataset), the audit logs are batched into smaller provenance graphs. In practice, a batch size of 250,000 edges is good enough to reduce memory consumption to an acceptable level without breaking important causal relationships between entities.

==> tex_section/model.tex <==
\section{Design Details}\label{sec_model}
In this section, we explain in detail how \system{} performs efficient APT detection from massive audit logs. \system{} contains four major components: a graph construction phase that builds optimised and consistent provenance graphs(Sec. \ref{sec_model_1}), a graph representation module that produces graph embeddings with maximum efficiency(Sec. \ref{sec_model_2}), a detection module that utilizes outlier detection methods to perform APT detection(Sec. \ref{sec_model_3}) and a model adaption mechanism to deal with \emph{concept drift} and other high-quality feedbacks(Sec. \ref{sec_model_4}).

\subsection{Provenance Graph Construction}\label{sec_model_1}

Data provenance transforms audit logs into a provenance graph to extract and present causal relationships between system entities. Based on data provenance, \system{} constructs a provenance graph out of raw audit logs before performing APT detection steps. As shown in figure \ref{fig_overview}, a prototype provenance graph can be constructed by simply extracting system entities as graph nodes and log entries as edges. However, two problems emerge during this construction process: (1) the enormous size of audit logs make the provenance graph too large to process(e.g. 6,113,983 nodes and 22,161,538 edges in DARPA TRACE dataset). (2) periodical interactions between system entities(e.g. network traffic) are often recorded as continuous block of log entries, creating hundreds even thousands of redundant edges. To address these problems, \system{} takes three steps to obtain a consistent and optimized provenance graph while keeping the valuable semantics intact: noise reduction to remove redundant and useless information, attribute extraction to abstract attributes of entities and interactions into labels and feature construction to generate raw feature vectors of nodes and edges. Detailed description of our graph construction steps are discussed in Appendix \ref{appe_a}.
After conducting the above three steps, \system{} has finished constructing a consistent and information-preserving provenance graph ready for subsequent tasks. During provenance graph construction, little information is lost as \system{} only damages the original semantics by generalizing detailed descriptions of system entities and interactions into labels. However, an average 52.90\% of all edges are reduced on the DARPA TRACE dataset, saving \system{}'s training time and memory consumption.

\subsection{Graph Representation Module}\label{sec_model_2}

\input{tex_figure/fig_gmae.tex}
\system{} employed a graph representation module to obtain high-quality graph embeddings from featured provenance graphs. As illustrated in Figure \ref{fig_gmae}, the graph representation module consists of three phases: an embedding layer that embeds the raw feature of nodes and edges into initial embedding vectors(Sec. \ref{sec_model_2_1}), a graph encoder that produces node and graph embeddings by propagating and aggregating graph features(Sec. \ref{sec_model_2_1}), a graph decoder that provides supervision signals to the training of the graph representation module via masked feature reconstruction and sample-based structure reconstruction(Sec. \ref{sec_model_2_3}). The encoder and decoder form a \emph{graph masked auto-encoder}, which excels in producing fast and resource-saving graph embeddings.

\subsubsection{Embedding Layer}\label{sec_model_2_1}

The function of the embedding layer is to transform one-hot features of both nodes and edges into high-dimensional fixed-length embeddings. For the sake of minimum computation overhead, we employed a simple \emph{lookup embedding} that establishes a one to one mapping between attributes and a vocabulary of embeddings. The vocabulary is a randomly initialized matrix of size $c\times d$, where $c$ is the dimension of attributes and $d$ is the hidden dimension of the graph representation module. Node and edge embeddings are obtained by simply looking up the corresponding column in the vocabulary with respect to the raw features.

Another function of the embedding layer is to perform \emph{masking} on nodes, so that the graph masked auto-encoder can be trained upon reconstruction of these nodes. Masked nodes are randomly chosen, covering a certain proportion of all nodes. The embeddings of such masked nodes are replaced with a special masked token $v_{mask}$ to cover any original information about these nodes. Edges, however, are not masked because these edges provide precious information about causal relationships between system entities. In summary, given node attributes $x_n$ and edge attributes $x_e$, the embedding layer produces node and edge embeddings from the vocabulary:
$$
\begin{aligned}
\begin{split}
emb_{n} &= \left\{
\begin{array}{ll}
v_i \in V_n, & {n \notin \widetilde{N}}\\
v_{mask}, & {n \in \widetilde{N}}
\end{array}
\right.\\
s.t.\ key(i) &= x_n\\
emb_{e} &= v_i \in V_e \\
s.t.\ key(i) &= x_e
\end{split}
\end{aligned}
$$
where $\widetilde{N}$ are masked nodes, $emb_n, emb_e \in R^d$ are node and edge embeddings and $V_n \in R^{c_n \times d}, V_e \in R^{c_e \times d}$ are vocabularies of such embeddings respectively.

\subsubsection{Graph Encoder}\label{sec_model_2_2}

Node embeddings produced by the embedding layer take only raw features into consideration. However, raw features are far from enough to model detailed behaviors of system entities. Contextual information of an entity, such as its neighborhood, its multi-hop causal relationships and its interaction patterns with other system entities plays an important role to obtain high-quality entity embeddings\cite{gin-28}. Here we employed and extended graph masked auto-encoders\cite{gmae-19} to generate node embeddings in a self-supervised way. The graph masked auto-encoder consist of an encoder and a decoder. The encoder produces node embeddings by propagating and aggregating graph features and the decoder reconstructs graph features to provide supervision signals for training. Such encoder-decoder architecture maintains the contextual and semantic information within the generated embeddings, while its computation overhead is significantly reduced via masked learning.

To explain in detail, the encoder of our graph representation module contains multiple stacked layers of graph attention networks(GAT)\cite{gat-29}. One layer of GAT takes node embeddings generated by previous layers as input, propagates and aggregates information from neighboring nodes and edges to update node embeddings. We also apply a three-way additive multi-head attention mechanism to assign importance factor to each neighbor. The aggregation function presented in our encoder is a GAT-style aggregation with residual connection. Overall, one GAT layer performs the following operation:
$$
\begin{aligned}
\alpha(src, dst) &= LeakyReLU(W_s^Th_{src}+W_e^Temb_{e}+W_d^Th_{dst}),\\
a(src, dst) &= Softmax(\alpha(src, dst)),\\
AGG(h_{src}, h_{\mathcal{N}}) &= W_{src}h_{src} + \sum_{i\in \mathcal{N}}a(src, i)W_{dst}h_i,\\
h_n^l &= AGG^l(h_n^{l-1}, h_{\mathcal{N}_n}^{l-1}),
\end{aligned}
$$
where $h_n^l$ is the hidden embedding of node $n$ at $l$-th layer of GAT, $h_n^{l-1}$ is that of layer $l-1$ and $\mathcal{N}_n$ is the one-hop neighborhood of $n$. The input of the first GAT layer is the original node embedding $emb_n$ obtained from provenance graph construction. $emb_e$ is the embedding of the edge and $a(src, dst)$ is the attention score between $src$ and $dst$. $W_s,W_e,W_d, W_{src},W_{dst}\in R^{d}$ are trainable parameters. 

Multiple layers of such graph attention networks are stacked to obtain the final node embeddings $h$, which is concatenated by the original node embedding and outputs of all GAT layers:
$$
\begin{aligned}
h_n = emb_n || h_n^1 || \cdots || h_n^l.
\end{aligned}
$$
where $\cdot||\cdot$ denotes the concatenate operation. Through stacked layers of GATs, the graph encoder effectively incorporates node attributes, multi-hop interaction and neighborhood information to abstract system entity behaviors into node embeddings. The graph encoder also applies an average pooling to all node embeddings to generate a comprehensive embedding of the graph itself\cite{graphpooling-30}, which recapitulates the overall state of the system:
$$
h_G = \frac{1}{|N|}\sum_{n_i\in N}h_{n_i}.
$$
where $N$ is the set of nodes in the provenance graph $G$. The node embeddings and system state embeddings generated by the graph encoder are considered the output of the graph representation module, which are used in subsequent tasks in different scenarios.

\subsubsection{Graph Decoder}\label{sec_model_2_3}

The graph encoder generates only graph embeddings and does not provide supervision signals that support model training. In typical graph auto-encoders\cite{vgae-24,gate-26}, a graph encoder is employed to decode node embeddings and supervise model training via \emph{feature reconstruction} and \emph{structure reconstruction}. Graph masked auto-encoders, however, abandon structure reconstruction to reduce computation overhead. Our graph decoder is a mixture of both, which integrates masked feature reconstruction and sample-based structure reconstruction to construct an objective function that optimizes the graph representation module.

Given node embeddings $h_n$ obtained from the graph encoder, the decoder first re-mask those masked nodes with the masked token $v_{mask}$. Then, a linear transformation is conducted on node embeddings to obtain the input of \emph{masked feature reconstruction}:
$$
\begin{aligned}
\begin{split}
h^*_n &= \left\{
\begin{array}{ll}
W^*h_n, & {n \notin \widetilde{N}}\\
W^*v_{remask}, & {n \in \widetilde{N}}
\end{array}
\right.,\\
\end{split}
\end{aligned}
$$
Subsequently, the decoder uses a similar GAT layer as described in the previous section to reconstruct the raw feature of the masked nodes. The reconstructed features have the same dimension as their raw features, which allows the calculation of a feature reconstruction loss:
$$
\begin{aligned}
x^*_n &= AGG^*(h^*_n, h^*_{\mathcal{N}_n}),\\
L_{fr} &= \frac{1}{|\widetilde{N}|}\sum_{n_i\in \widetilde{N}}(1-\frac{x_{n_i}^Tx^*_{n_i}}{||x_{n_i}||\cdot||x^*_{n_i}||})^\gamma.
\end{aligned}
$$
where $L_{fr}$ is the masked feature reconstruction loss obtained by calculating a \emph{scaled cosine loss} between raw and reconstructed features of the masked nodes. Such loss\cite{gmae-19} scales dramatically between easy and difficult samples which effectively speeds up learning. The degree of such scaling is controlled by a hyper-parameter $\gamma$.

The sample-based structure reconstruction, on the other hand, aims to reconstruction graph structure(i.e. predict edges between nodes). Instead of reconstructing the whole adjacency matrix, which has $O(N^2)$ complexity, sample-based structure reconstruction apply contrastive sampling on node pairs and predict edge probabilities between such pairs. Only non-masked nodes are involved in structure reconstruction. Positive samples are constructed with all existing edges between non-masked nodes and negative samples are sampled among node pairs with no existing edges between them.

A simple two-layer MLP is used to reconstruct edges between sampled node pairs, generating a probability for each sample. The reconstruction loss takes the form of a simple binary cross-entropy loss on those samples:
$$
\begin{aligned}
prob(n, n') &= \sigma(MLP(h_n||h_{n'})),\\
L_{sr} = -\frac{1}{|\hat{N}|}\sum_{n\in \hat{N}}(&log(1-prob(n,n^-))+log(prob(n,n^+))).
\end{aligned}
$$
where $(n,n^-)$ and $(n,n^+)$ are negative and positive samples respectively and $\hat{N}=N - \widetilde{N}$ is the set of non-masked nodes. The sample-based structure reconstruction only provides supervision to the graph embeddings. Instead of using dot products, we employ a MLP to calculate edge probabilities as interacting entities are not necessarily similar in behaviors. Also, we are not forcing the model to learn to predict edge probabilities. The function of such structure reconstruction is to \emph{maximize behavioral information} contained in the abstracted node embeddings so that a simple MLP is sufficient to incorporate and interpret such information into edge probabilities.

The final objective function $L = L_{fr} + L_{sr}$ combines the masked feature reconstruction and sample-based structure reconstruction provides supervision signals to the graph representation module, enabling it to learn parameters in a self-supervised way.
\subsection{Detection Module}\label{sec_model_3}

Based on the graph embeddings generated by the graph representation module, we utilize outlier detection methods to perform APT detection in an unsupervised way. As detailed explained in previous sections, such embeddings summarize system behaviors in different granularity. The goal of our detection model, is to identify malicious system entities or states given only a priori knowledge of \emph{benign system behaviors}. Embeddings generated via graph representation learning tend to form clusters if their corresponding entities share similar interaction behaviors in the graph\cite{gate-26, gala-25,vgae-24,gmae-19,heco-32}. Thus, outliers in graph embeddings indicate uncommon and suspicious system behaviors. Based on such insight, we develop a special outlier detection method to perform APT detection. 

During training, benign embeddings are first abstracted from the training provenance graphs. What the detection module do at this stage is simple \emph{memorizing} those embeddings and organize them in a special data structure called a \emph{K-D Tree}\cite{kdtree-33} optimized for nearest neighbor search. After training, the detection module reveals outliers in three steps: k-nearest neighbor searching, similarity calculation and filtering. Given a target embedding, the detection module first obtains its k-nearest neighbors via K-D Tree searching. Such searching process only takes $log(N)$ time, where $N$ is the total number of memorized training embeddings. Then, a similarity criterion is applied to the target embedding and its neighbors to evaluate its closeness to benign embeddings. Such closeness measurement is further transformed into an anomaly score. If its anomaly score yields higher than a hyper-parameter $\theta$, the target embedding is considered an outlier and its corresponding system entity or system state is malicious. An example workflow of the detection module is formalized as follows, using euclidean distance as the similarity criterion:
$$
\begin{aligned}
\begin{split}
\mathcal{N}_x &= KNN(x)\\
dist_x &= \frac{1}{|\mathcal{N}_x|}\sum_{x_i\in \mathcal{N}_x}||x-x_i||\\
score_x &= \frac{dist_x}{\overline{dist}}\\
result_x &= \left\{
\begin{array}{ll}
1, & score_x\geq\theta\\
0, & score_x<\theta
\end{array}
\right.\\
\end{split}
\end{aligned}
$$
where $\overline{dist}$ is the average distance between training embeddings and their k-nearest neighbors. When performing \emph{batched log level detection}, the detection module memorizes benign system state embeddings that reflects system states and detect if the system state embedding of a newly-arrived provenance graph is an outlier. When performing \emph{system entity level detection}, the detection module instead memorizes benign \emph{node embeddings} that indicates system entity behaviors and given a newly-arrived provenance graph, it detect outliers within the embeddings of all system entities. 

\subsection{Model Adaption}\label{sec_model_4}
When constructing an APT detector, especially those applied to real-world detection scenarios, concept drift must be taken into consideration. When facing benign yet previously unseen system behaviors, \system{} produces false positive detection results, which may mislead subsequent applications, e.g. attack investigation and story recovery. Recent works address this issue by forgetting outdated data\cite{aptlearnbased-10} or fitting their model to benign system changes via a \emph{model adaption mechanism}\cite{aptlearnbasedshadewatcher-18}. \system{} also integrate a model adaption mechanism to combat concept drift and help the model to learn from false positives identified by security analysts. Slightly different from other works that use only false positives to retrain the model, \system{} can be retrained with all feedbacks. As discussed in previous sections, the graph representation module in \system{} encodes system entities into embeddings in a self-supervised way, without knowing its label. Any unseen data, including those true negatives, are valuable training data for the graph representation module to enhance its representation ability on unseen system behaviors. 

The detection module can only be retrained with benign feedbacks to keep up to system behavior changes. And as it memorizes more and more false positive feedbacks, its detection efficiency is lowered. To address this issue, we also implement a discounting mechanism on the detection module. When the volume of memorized embeddings exceeds a certain amount, earliest embeddings are simply removed as newly-arrived embeddings are learned. While low-quality feedbacks\cite{aptlearnbasedshadewatcher-18} have an enormous impact on our detection module and poison attacks may penetrate \system{} via model adaption, we provide the model adaption mechanism as an optional solution to concept drift and unseen system behaviors. It is recommended to adapt \system{} to system changes with newly-obtained benign audit logs only. 
















==> tex_section/motivation.tex <==
\section{Background}

\subsection{Motivating Example}\label{sec_motivation_1}
Here we provide a detailed illustration of an APT scenario that we use throughout the paper. Pine backdoor with drakon dropper is an APT attack from the DARPA TRACE dataset\cite{darpadataset-20}. During the attack, an attacker constructs a malicious executable(\emph{/tmp/tcexec}) and sends it to the target host via a phishing e-mail. The user then unconsciously downloads and opens the e-mail. Contained within the e-mail is an executable designed to perform a port-scan for internal reconnaissance and establish a silent connection between the target host and the attacker. Figure \ref{fig_motivation} displays the provenance graph of our motivation example. Nodes in the graph represent system entities and arrows represent directed interactions between entities. The graph shown is a subgraph abstracted from the complete provenance graph by removing all attack-irrelevant entities and interactions. Different node shape corresponds to different type of entities. Entities and interactions marked red are considered malicious ones.

\input{tex_figure/fig_motivation.tex}
\subsection{Prior Research and their Limitations}\label{sec_motivation_2}

\noindent\textbf{Supervised Methods.} For early works\cite{aptrulebased-2,aptrulebased-4,aptrulebasedholmes-3,aptrulebased-5,aptrulebased-6}, special heuristic rules need to be constructed to cover all attack patterns. Many DL-based APT detection methods\cite{aptlearnbasedatlas-11,aptlearnbased-14,aptlearnbasedprovgem-15,aptlearnbased-16,aptlearnbasedshadewatcher-18} construct provenance graphs based on both benign and attack-containing data and detect APTs in a classification style. These supervised methods can achieve almost perfect detection results on learned attack patterns but are especially vulnerable facing \emph{concept drift} or unseen attack patterns. Moreover, for rule-based methods, the construction and maintenance of heuristic rules is very expensive and time-consuming. And for DL-based methods, the scarcity of attack-containing data is preventing these supervised methods from being actually deployable. To address the above issue, \system{} adopts a fully self-supervised anomaly detection style, allowing the absence of attack-containing data while effectively dealing with unseen attack patterns. 

\noindent\textbf{Statistics-based Methods.} Most recent statistics-based methods\cite{aptstatbasednodoze-7,aptstatbased-8,aptstatbased-9} detect APT signals by identifying system entities, interactions and communities based on their rarity or anomaly scores. However, the rarity of system entities may not necessarily indicate their abnormality and anomaly scores, obtained via causal analysis or label propagation, are \emph{shallow feature extraction} on provenance graphs. To illustrate, the process \emph{tcexec} performs multiple portscan operations on different IP addresses in our motivating example(See Figure \ref{fig_motivation}), which may be considered as a normal system behavior. However, taking into consideration that process \emph{tcexec}, derived from the external network, also reads sensitive system information(\emph{uname}) and makes connection with public IP addresses(\emph{162.66.239.75}), we can easily identify \emph{tcexec} as a malicious entity. Failure to extract deep semantics and correlations between system entities often results in low detection performance and high false positive rate of statistics-based methods. \system{}, however, employs a graph representation module to perform \emph{deep graph feature extraction} on provenance graphs, resulting in high-quality graph embeddings.

\noindent\textbf{DL-based Methods.} Recently, ML-based APT detection methods, no matter supervised or unsupervised, are producing very promising detection results. However, in reality, hundreds of GB of audit logs are produced every day in a medium-size enterprise\cite{datascale-23}. Consequently, ML-based methods, especially sequence-based\cite{aptlearnbasedatlas-11,aptlearnbased-14} and graph-based\cite{aptlearnbased-10,aptlearnbased-12,aptlearnbasedprovgem-15,aptlearnbased-16,aptlearnbasedthreatrace-17,aptlearnbasedshadewatcher-18} methods, are impracticable due to their computation overhead. For instance, ATLAS\cite{aptlearnbasedatlas-11} takes an average 1 hour to train on 676MB of audit logs and ShadeWatcher\cite{aptlearnbasedshadewatcher-18} takes 1 day to train on the DARPA TRACE dataset with GPU available. Besides, Some graph auto-encoder\cite{vgae-24,gala-25,gate-26} based methods encounter \emph{explosive memory overhead} problem when the scale of provenance graphs expands. \system{} avoids to be computationally demanding by introducing \emph{graph masked auto-encoders} and completes its training on the DARPA TRACE dataset in just several minutes. Detailed evaluation of \system{}'s performance overhead is discussed in Sec. \ref{sec_evaluation_5}.

\noindent\textbf{End-to-end Approaches}. Beyond the three major limitations discussed above, it is also worth to mention that most recent APT detection approaches are \emph{end-to-end} detectors and focus on one specific detection task. Instead, \system{}'s approach is universal and performs multi-granularity APT detection under various detection scenarios, which also applies to audit logs come from different sources. 

\subsection{Threat Model and Definitions}\label{sec_definition}
We first present the threat model we used throughout the paper and then formally define key concepts that are crucial to understanding how \system{} performs APT detection.

\noindent\textbf{Threat Model.} We assume that APT attacker comes from outside a system and target valuable data within the system. The attacker may perform sophisticated steps to achieve his goal but leave trackable evidence in system audit logs. The combination of the system hardware, operating system and system audit softwares is our trusted computing base and poison attacks that attempts to corrupt the APT detection system before attacking is considered in our threat model.

\noindent\textbf{Provenance Graph.} Data provenance transform raw audit logs into the form of a directed graph. Such graph is called a \emph{provenance graph} as nodes in a provenance graph represent system entities and edges between those entities indicate causal relationships between them. Here we denote a provenance graph as $G=\{N,E\}$, where $N=\{n_1, n_2,...n_n\}$ is the set of nodes and $E=\{(src, dst)|src,dst\in N\}$ is the set of edges in the graph. Nodes and edges in the provenance graph have types which can be easily extracted from the original audit logs. For example, \emph{/tmp/tcexec} is a system entity of type \emph{FileObject} and the interaction between \emph{/tmp/tcexec} and \emph{tcexec} is an \emph{execute} operation from a \emph{FileObject} targeting a \emph{Process}, as illustrated in Figure \ref{fig_motivation}. 

\noindent\textbf{Multi-granularity Detection.} \system{} is capable to perform APT detection at two-granularity: \emph{batched log level} and \emph{system entity level}.

\vspace{3pt}\noindent$\bullet$~ Batched log level detection. Under this granularity of APT detection, the major task is \emph{given batched audit logs from a consistent source, \system{} alerts if a potential APT is detected in a batch of logs}. Similar to Unicorn\cite{aptlearnbased-10}, \system{} does not accurately locate malicious system entities and interactions under this granularity of detection.

\vspace{3pt}\noindent$\bullet$~ System entity level detection. The detection task under this granularity of APT detection is \emph{given audit logs from a consistent source, \system{} is able to accurately locate malicious system entities in those audit logs}. Identification of key system entities during APTs is vital to subsequent tasks such as attack investigation and attack story recovery as it provides explicable detection results and reduces the need for domain experts as well as redundant manual efforts\cite{aptlearnbasedatlas-11}.

==> tex_section/overview.tex <==
\input{tex_figure/fig_overview.tex}
\section{\system{} Overview}

\system{} is a novel self-supervised APT detection approach that leverages masked graph representation learning and outlier detection methods and is capable of efficiently performing multi-granularity detection on massive audit logs. \system{}'s pipeline consists of three main components: (1) provenance graph construction, (2) a graph representation module and (3) a detection module. It also provides an optional (4) model adaption mechanism. During training, \system{} transforms training data with (1), learns graph embedding by (2) and memorizes benign behaviors in (3). During inference, \system{} transforms target data with (1), obtain graph embedding with the trained (2) and detects outliers through (3). Figure \ref{fig_overview} gives an overview of the \system{} architecture.

During provenance graph construction(1), audit logs collected by system auditing softwares are transformed into provenance graph(s). System entities and interactions between them are extracted and converted into attributed nodes and edges respectively. Several complexity reduction techniques, such as noise reduction\cite{aptlearnbasedshadewatcher-18}, are integrated into the graph construction process to remove redundant information and keep the provenance graph consistent.

The constructed provenance graphs are then fed through the graph representation module to obtain graph embeddings(i.e. comprehensive vector representations of objects)(2). Built upon \emph{graph masked auto-encoders} and integrates \emph{sample-based structure reconstruction}, the graph representation module embeds, propagates and aggregates node and edge attributes into graph embeddings, which contain both node embeddings and the system state embedding. 

The graph representation module is trained with only benign audit logs to model benign system behaviors. When performing APT detection on potentially attack-containing audit logs, \system{} utilizes \emph{outlier detection methods} based on the graph embeddings to detect outliers in system behaviors(3). Depending on the granularity of the task, different embeddings are used to complete APT detection. When performing \emph{batched log level detection}, the system state embeddings, which reflect the general behaviors of the whole system, are the targets of outlier detection. An outlier in such embeddings means its corresponding system state is unseen and potentially malicious, which reveals an APT signal in that batch of audit logs. When performing \emph{system entity level detection}, the detection targets are those node embeddings, which represent the behaviors of system entities. Outliers in node embeddings, however, indicates suspicious system entities and detects APT threats in finer granularity.

To deal with \emph{concept drift}, stealth attacks and unseen attacks, an optional model adaption mechanism is employed to provide feedback channels for its users(4). Detection results that are confirmed by security analysts are fed back to \system{}, helping it to adapt to benign system behavior changes in a semi-supervised way.

\system{} is designed to perform offline APT detection under unsupervised or semi-supervised conditions. However, under fully supervised conditions, \system{} achieves even more promising detection results, which is discussed in Sec. \ref{sec_evaluation_4}. Furthermore, \system{} can be easily applied to real-world online APT detection thanks to it's ability to adapt itself to \emph{concept drift} and its minimum computation overhead.









==> tex_section/related.tex <==
\section{Related Work}

\system{} is mainly related to three fields of research, including the detection of APTs, graph representation learning and outlier detection methods.

\noindent\textbf{APT Detection.} The goal of APT detection is given audit logs collected by system auditing softwares, detect APT signals, malicious entities and invalid interactions between entities. Recent works on APT detection are based on data provenance. As suggested by \cite{aptlearnbasedshadewatcher-18}, provenance-based detectors can be categorized into rule-based, statistics-based and learning-based approaches. Rule-based approaches\cite{aptrulebased-2,aptrulebasedholmes-3,aptrulebased-4,aptrulebased-5,aptrulebased-6} utilize \emph{a priori} knowledge about previous seen APT attacks and construct unique heuristic rules for detecting them. Statistics-based approaches\cite{aptstatbased-8,aptstatbased-9,aptstatbasednodoze-7} construct statistics to measure the abnormality of provenance graph elements and perform anomaly detection on them. Learning-based approaches\cite{aptlearnbased-10,aptlearnbasedatlas-11,aptlearnbased-12,atplearnbased-13,aptlearnbased-14,aptlearnbasedprovgem-15,aptlearnbased-16,aptlearnbasedthreatrace-17,aptlearnbasedshadewatcher-18} use deep learning to model either benign system behaviors\cite{aptlearnbased-10,aptlearnbased-12,aptlearnbasedthreatrace-17} or attack patterns\cite{aptlearnbasedatlas-11,aptlearnbased-14,aptlearnbasedprovgem-15,aptlearnbased-16,aptlearnbasedshadewatcher-18} and perform APT detection as classification\cite{aptlearnbasedatlas-11,aptlearnbasedprovgem-15,aptlearnbased-16} or anomaly detection\cite{aptlearnbasedshadewatcher-18}. These approaches are further divided into sequence-based and graph-based methods. Sequence-based methods\cite{aptlearnbasedatlas-11,aptlearnbased-14} model system executions and detect APTs based on their workflow patterns. Graph-based methods\cite{aptlearnbased-10,aptlearnbased-12,aptlearnbasedprovgem-15,aptlearnbased-16,aptlearnbasedthreatrace-17,aptlearnbasedshadewatcher-18} model system entities and the system state via GNNs and their primitive variants and detect APTs based on abnormal behaviors.

\noindent\textbf{Graph Representation Learning.} Embedding techniques on graphs start from the graph convolutional network(GCN)\cite{gcn-51} and is further enhanced by the graph attention network(GAT)\cite{gat-29} and GraphSAGE\cite{graphsage-52}. While these techniques are mainly supervised, graph auto-encoders\cite{vgae-24,gala-25,gate-26,gmae-19} bring unsupervised solutions for graph representation learning. GAE, VGAE\cite{vgae-24} and GATE\cite{gate-26} utilize feature reconstruction and structure reconstruction(i.e. adjacency matrix reconstruction) to learn graph embeddings in a self-supervised way. However, they focus on link prediction and graph clustering tasks, irrelevant to our application. Recently, graph masked auto-encoders\cite{gmae-19} leverages masked feature reconstruction and achieved state-of-the-art results on various applications with minimum overhead.

\noindent\textbf{Outlier Detection.} Outlier detection methods view outliers(i.e. objects that may not belong to the ordinary distribution) as anomalies and aim to identify them. Traditional outlier detection methods are One-class SVMs\cite{ocsvm-47}, Isolation Forest\cite{if-48} and Local Outlier Factor\cite{lof-53}. Many anomaly detection approaches successfully apply these outlier detection methods to various detection scenarios, including credit card fraud detection\cite{ocan-55}, abnormal community detection\cite{community-56} and malicious transaction detection\cite{transaction-57}. This proves that outlier detection methods work well to detect malicious targets in different scenarios. Besides, auto-encoders themselves are effective tools for outlier detection. We explain why graph auto-encoders cannot detect anomalies in our provenance graphs in Appendix \ref{appe_d}.

==> tex_section_revised/implementation_backup.tex <==
\section{Implementation}\label{sec_implementation_revised}

We implement \system{} with about 3,500 lines of code in Python 3.8. We developed several log parsers to cope with different format of audit logs, including a simple StreamSpot format\cite{streamspot-35} and more complex ones such as Camflow\cite{camflow-34}and CDM\cite{cdm-36}. Provenance graphs are constructed using the graph processing library Networkx\cite{networkx-37}. Those provenance graphs are generated and stored into an universal JSON format for the sake of compatibility. The graph representation module is implemented via PyTorch\cite{pytorch-38} and the DGL library\cite{dgl-40} and the detection module is developed with Scikit-learn\cite{sklearn-39}. An Adam optimizer with the weight decay factor equals $5\times10^{-4}$ is used to optimize the graph representation module.

For hyper-parameters of MAGIC, the scaling factor $\gamma$ in the feature reconstruction loss is set to 3, the number of neighbors k is set to 10 and the learning rate set to 0.001. We use a 3 layer graph encoder and a mask rate of 0.5 in our experiments. The output embedding dimension d is different on two detection scenarios, batched log level detection and entity level detection. We use d equals 256 in batched log level detection and of and an we set d equals 64 in entity level detection to reduce resource consumption. The hyper-parameters may have other choices, like the dimension d of output embeddings can be chosen from \{16, 32, 64, 128, 256\} and beyond, the number of GAT layers l in the graph encoder from \{1, 2, 3, 4\}, the mask rate of nodes from \{0.3, 0.5, 0.7\}. The detection threshold $\theta$ is chosen by a simple linear search separately conducted on the two different scenarios. In batched log level detection, $\theta$ is chosen between 1 and 10. In entity level detection, $\theta$ is searched between 1000 and 6500.  We demonstrate the impact of these hyper-parameters on MAGIC later in the evaluation section. 

==> tex_table/tab_ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\belowcaptionskip}{0.2cm}
\caption{Effect of masked feature reconstruction and sample-based structure reconstruction in \system{}'s graph representation model, evaluated on the Wget dataset.}
\label{tab_ablation}

\begin{tabular}{|c|c|c|c|}

\hline
Model & F1-Score & Overhead\\
\hline\hline

No FR & 68\% & 44.9\%\\
\hline

Ordinary FR (baseline)& 96\% & 100.0\%\\
\hline

\textbf{Masked FR (Ours)}& 97\% & 54.1\%\\
\hline\hline

No SR & 89\% & 6.9\%\\
\hline

Full SR (baseline)& 97\% & 100.0\% \\
\hline

\textbf{Sample-based FR (Ours)} & 97\% & 9.9\% \\
\hline
\end{tabular}
\end{table}


==> tex_table/tab_avg_distance.tex <==
\begin{table}[t]
\centering
\small
\setlength{\belowcaptionskip}{0.2cm}
\caption{Average distance between malicious target embeddings and benign ones (i.e. anomaly scores), evaluated on all dataset.}
\label{tab_avg_distance}
\begin{tabular}{|c|c|c|c|}
\hline
Dataset & StreamSpot & \makecell[c]{DARPA\\TRACE} & \makecell[c]{Unicorn\\Wget} \\
\hline

Avg. anomaly score & 65.04 & 14.33 & 4.86\\
\hline
\end{tabular}
\end{table}

==> tex_table/tab_avg_distance_revised.tex <==
\begin{table}[t]
\centering
\small
\setlength{\belowcaptionskip}{0.2cm}
\caption{Average anomaly scores of malicious target embeddings, evaluated on all dataset. W}
\label{tab_avg_distance_revised}
\begin{tabular}{|c|c|c|c|}
\hline
Dataset & StreamSpot & \makecell[c]{DARPA\\E3 Trace} & \makecell[c]{Unicorn\\Wget} \\
\hline

Avg. anomaly score & 67.94 & 6606.07 & 11.26\\
\hline
\end{tabular}
\end{table}

==> tex_table/tab_compare_result.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Comparison between \system{} and state-of-the-art APT detection methods on different datasets. Within column \emph{supervision}, B indicates benign data, A refers to attack data and SA for streaming attack data.}
\label{tab_compare_result}

\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}

\hline
Dataset & Method & Train Ratio & Supervision & F1-Score & Recall & FPR\\
\hline\hline

\multirow{5}{*}{StreamSpot} & StreamSpot & 80\% & B & 81\% & 91\% & 6.6\%\\

 & Unicorn (baseline) & 75\% & B & 96\% & 93\% & 1.6\%\\

 & Prov-Gem & 80\% & B,A & 97\% & 94\% & N/A\%\\

 & ThreaTrace & 75\% & B & 99\% & 99\% & \textbf{0.4\%}\\

 & \textbf{\system{}(Ours)} & 80\% & B & \textbf{99\%} & \textbf{100\%} & 0.6\%\\
\hline\hline

\multirow{4}{*}{\makecell[c]{Unicorn\\Wget}} & Unicorn (baseline) & 80\% & B & 90\% & 95\% & 15.5\%\\

 & Prov-Gem & 80\% & B,A & 89\% & 80\% & N/A\%\\

 & ThreaTrace & 80\% & B & 95\% & \textbf{98\%} & 7.4\%\\

 & \textbf{\system{}(Ours)} & 80\% & B & \textbf{97\%} & 96\% & \textbf{2.0\%}\\
\hline\hline

\multirow{5}{*}{\makecell[c]{DARPA\\TRACE}} & DeepLog & N/A & B,A & 51\% & 68\% & 2.7\%\\

& Log2vec (baseline) & N/A & B,A & 64\% & 78\% & 1.8\%\\

& ThreaTrace & 69\% & B & 83\% & \textbf{99\%} & 1.1\%\\

& ShadeWatcher & 80\% & B,SA & \textbf{99\%} & 99\% & \textbf{0.3\%}\\

 & \textbf{\system{}(Ours)} & \textbf{20\%} & B & 99\% & 99\% & 0.5\%\\
\hline
\end{tabular}
}
\end{table}


==> tex_table/tab_entity_dataset.tex <==
\begin{table}[t]
\caption{Datasets for System Entity Level Detection.}
\label{tab_entity_dataset}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Dataset & Scenario & Malicious &\#Node &\#Edge & Size(GB)\\
\hline\hline
 \multirow{5}{*}{DARPA TRACE} & Benign & & 6,045,886 & \multirow{5}{*}{8,354,082} & \multirow{5}{*}{15.0}\\

 & Extension Backdoor & \checkmark & 732 & & \\

 & Firefox Backdoor & \checkmark & 8 & & \\

 & Pine Backdoor & \checkmark & 67,341 & & \\

 & Phishing Executable & \checkmark & 16 & & \\
 \hline
\end{tabular}
}
\end{table}


==> tex_table/tab_fpr.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{\system{}'s false positive rates on different datasets. The effect of model adaption mechanism is tested under different settings.}
\label{tab_fp_result}

\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}

\hline
Dataset & Train Ratio & Adaption & Test Ratio & FPR\\
\hline\hline

StreamSpot & 80\% & N/A & 20\% & 0.590\%\\
\hline

Unicorn Wget & 80\% & N/A & 20\% & 2.000\%\\
\hline

\multirow{5}{*}{\makecell[c]{DARPA\\TRACE}} & 20\% & N/A & 80\% & 0.509\%\\

& 20\% & N/A & 60\% & 0.520\%\\

& 20\% & 10\% FP & 60\% & 0.468\%\\

& 20\% & 20\% FP & 60\% & 0.402\%\\

& 20\% & 20\% FP \& TN & 60\% & 0.398\%\\
\hline
\end{tabular}}
\end{table}


==> tex_table/tab_general_result.tex <==
\begin{table*}[t]
\caption{\system{}'s detection results on different datasets. For batched log level detection, the detection targets are log pieces. And for system entity level detection, the detection targets are system entities.}
\label{tab_general_result}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|cccc|cccc|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Detection Granularity} & \multirow{2}{*}{Train Ratio} & \multicolumn{2}{c|}{Ground Truth} &\multirow{2}{*}{\#TP} &\multirow{2}{*}{\#FP} & \multirow{2}{*}{\#TN} & \multirow{2}{*}{\# FN} & \multirow{2}{*}{Precision} & \multirow{2}{*}{Recall} & \multirow{2}{*}{Accuracy} & \multirow{2}{*}{F1-Score}\\
\cline{4-5}

 & & & \#Benign & \#Malicious & & & & & & & &\\
\hline\hline
 
 StreamSpot & Batched log level detection & 80\% & 100 & 100 & 100.0 & 0.59 & 99.41 & 0.0 & 99.41\% & 100.00\% & 99.71\% & 99.71\%\\
\hline

 Unicorn Wget & Batched log level detection & 80\% & 25 & 25 & 24.0 & 0.5 & 24.5 & 1.0 & 98.02\% & 96.00\% & 97.00\% & 96.98\%\\
 \hline

 DARPA TRACE & System entity level detection & 20\% & 4,773,947 & 68,265 & 68,223.0 & 24,299.4 & 4,749,647.6 & 42.0 & 73.73\% & 99.94\% & 99.50\% & 84.86\%\\
\hline
\end{tabular}}
\end{table*}


==> tex_table/tab_overhead.tex <==
\begin{table}[t]
\centering
\setlength{\belowcaptionskip}{0.2cm}
\caption{Performance Overhead of \system{} on DARPA TRACE dataset.}
\label{tab_overhead}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Phase} & \multirow{2}{*}{Component} & \multicolumn{2}{c|}{Time consumption(s)} & \multirow{2}{*}{Memory consumption(MB)}\\
\cline{3-4}

& & with GPU & CPU only & \\

\hline\hline

\makecell[c]{Graph\\Construction} & N/A & 159 & 159 & 390\\
\hline

\multirow{2}{*}{Training} & \makecell[c]{Graph\\Representation} & 63 & 255 & 1,202\\

\cline{2-5}

& Detection & 61 & 61 & 676\\
\hline

\multirow{2}{*}{Inference} & \makecell[c]{Graph\\Representation} & 5 & 20 & 416\\

\cline{2-5}

& Detection & 2,499 & 2,499 & 453\\
\hline
\end{tabular}}
\end{table}
